On Relevant Equilibria in Reachability Games

We study multiplayer reachability games played on a finite directed graph equipped with target sets, one for each player. In those reachability games, it is known that there always exists a Nash equilibrium (NE) and a subgame perfect equilibrium (SPE). But sometimes several equilibria may coexist such that in one equilibrium no player reaches his target set whereas in another one several players reach it. It is thus very natural to identify "relevant" equilibria. In this paper, we consider different notions of relevant equilibria including Pareto optimal equilibria and equilibria with high social welfare. We provide complexity results for various related decision problems.

==> sv-NEcomplexity.tex <==
%!TEX root=sv-main.tex
\subsubsection{Complexity and memory results}


\begin{theorem}
	\label{thm:NEComplexity}
	Let $(\mathcal{G},v_0)$ be a quantitative reachability game, for NE: Problem~\ref{prob:decisionThreshold} and Problem~\ref{prob:decisionWelfare} are NP-complete while Problem~\ref{prob:decisionPareto} is NP-hard and belongs to $\Sigma^P_2$.	
\end{theorem}
	
	
\begin{theorem}
	\label{thm:NEMemory}
		Let $(\mathcal{G},v_0)$ be a quantitative reachability game and for NE: \emph{(i)} for each decision problem, if its answer is positive, then there exists a strategy profile $\sigma$ with memory in  $\mathcal{O}((|\Pi|+1)\cdot |V| + |\Pi|)$ which satisfies the constraints{\color{red}/problem}, \emph{(ii)} for Problem~\ref{prob:decisionThreshold}, $\sigma$ is such that: if $i \in \Visit(\outcome{\sigma}{v_0})$, $\Cost_i(\outcome{\sigma}{v_0}) \leq |\Pi|\cdot|V|$ and \emph{(iii)} for Problem~\ref{prob:decisionWelfare}, $\sigma$ is such that: $\sum_{i \in \Visit(\outcome{\sigma}{v_0})} \Cost_i(\outcome{\sigma}{v_0}) \leq |\Pi|^2 \cdot |V|$.
\end{theorem}
	

% \begin{theorem}[Threshold decision problem]
% 	\label{thm:NEThreshold}
% 	Let $(\mathcal{G},v_0)$ be a qualitative/quantitative reachability game. 
% 	\begin{itemize}
% 		\item For NE, Problem~\ref{prob:decisionThreshold} is NP-complete.
% 		\item If the answer to this decision problem is affirmative, then there exists a strategy profile $\sigma$ with memory in  $\mathcal{O}((|\Pi|+1)\cdot |V| + |\Pi|)$ which satisfies the constraints. Additionnaly, for quantitative reachability games $\sigma$ is such that $\Cost_i(\outcome{\sigma}{v_0}) \leq |\Pi|\cdot|V|$ if $i \in \Visit(\outcome{\sigma}{v_0})$.
% 		%\item The strategy profile which satisfies constraints of~\eqref{item:compConstExistProb3} need at most $ \max_{i\in\Pi} \{ \overline{y_i} \mid \overline{y_i} < +\infty \} + |V| + |\Pi|$ memory.
% 	\end{itemize}
% \end{theorem}
% 
% Notice that, for the quantitative setting, this result also means that if we want to decide if there exists an NE such that Player $i$ visits his target set -- it is like chosing $< +\infty$ for the threshold of Player $i$ -- it suffies to decide this existence with the threshold $|\Pi| \cdot |V|$ for Player $i$.
% 
% \begin{theorem}[Social welfare decision problem]
% 	\label{thm:NEWelfare}
% 	Let $(\mathcal{G},v_0)$ be a qualitative/quantitative reachability game. 
% 	\begin{itemize}
% 		\item For NE, Problem~\ref{prob:decisionWelfare} is NP-complete.
% 		\item If the answer to this decision problem is positive, then there exists a strategy profile $\sigma$ with memory in  $\mathcal{O}((|\Pi|+1)\cdot |V| + |\Pi|)$ which satisfies the constraints. Additionnaly, for quantitative reachability games, $\sigma$ is such that $\sum_{i \in \Visit(\outcome{\sigma}{v_0})} \Cost_i(\outcome{\sigma}{v_0}) \leq |\Pi|^2 \cdot |V|$ . 
% 	\end{itemize}
% \end{theorem}
% 
% \begin{theorem}[Pareto optimality decision problem]
% 	\label{thm:NEPareto}
% 	
% 	Let $(\mathcal{G},v_0)$ be a qualitative/quantitative reachability game,
% 	
% 	\begin{itemize}
% 		\item For NE, Problem~\ref{prob:decisionPareto} is NP-hard and belongs to $\Sigma^P_2$.
% 		\item If the answer to this decision problem is positive, then there exists a strategy profile $\sigma$ with memory in  $\mathcal{O}((|\Pi|+1)\cdot |V| + |\Pi|)$ which satisfies the problem.
% 	\end{itemize}
% \end{theorem}










==> sv-appNE.tex <==
%!TEX root=sv-main.tex
\section{Complements of Section~\ref{section:resOnNE}}
\label{app:resNE}


%--------
%\input{sv-appCorollary1}

%----NE-Threshold

\subsection{Proof of Theorem~\ref{thm:NEComplexity} and Theorem~\ref{thm:NEMemory} for Problem~\ref{prob:decisionThreshold}}


% We now give a sketch of proof for the results in the qualitative setting.
% 
% \begin{proof}[Sketch of proof of Theorem~\ref{thm:NEThreshold} for qualitative reachability games]
% 
% It is summarized in~\cite{Bruyere17} that Problem~\ref{prob:decisionThreshold}  for quantitative reachability games is NP-complete for Nash equilibrium. To our knowledge, there is no explicit result about the memory which is needed to satisfy the constraints of this problem. We can find the same kind of result as previously. The characterization of the outcomes of NEs can be used by replacing cost functions by gain functions, inversing the inequality and using values in qualitative coalitional games in place of the quantitative ones. Moreover, as applying procedure (P1) on an outcome does not change the gain in the new outcome, the discussion we did in Remark~\ref{rem:twoThresholds} is not needed in this case. Thus, we can use exactly the same arguments  as before to state that if there exists an NE which satisfies the constraints then there exists an other one which satisfies the constraints too but with memory in $\mathcal{O}((|\Pi|+1)\cdot |V| + |\Pi|)$. \qed
% \end{proof}


%---
\subsection{Proof of Theorem~\ref{thm:NEComplexity} and Theorem~\ref{thm:NEMemory} for Problem~\ref{prob:decisionWelfare}}



%-----
\subsection{Proof of Theorem~\ref{thm:NEComplexity} and Theorem~\ref{thm:NEMemory} for Problem~\ref{prob:decisionPareto}}


{\color{red} PREUVE DE DURETE}




==> sv-appWitness.tex <==
%!TEX root=sv-main.tex
\section{Complements to Section~\ref{subsection:SPE}}
\label{app:witness}






%-----
\subsection{Proof of Theorem~\ref{thm:SPEMemory} for Problem~\ref{prob:decisionThreshold} in quantitative reachability games}





\subsection{Proof of Theorem~\ref{thm:SPEComplexity} and Theorem~\ref{thm:SPEMemory} for Problem~\ref{prob:decisionWelfare}}







==> sv-componentWise.tex <==
%!TEX root=sv-main.tex
\subsubsection{Threshold decision problem}

% Thanks to previous works and results in the sequel of this document, we obtain the results sumarized in Table~\ref{tab:resCompConstProb}.
% 
% 
% 
% \begin{table}[!ht]
% 	
% \label{tab:resCompConstProb}
% \caption{Results for Problem~\ref{prob:decisionThreshold}.}
% \centering
% \scalebox{0.8}{\begin{tabular}{|l|c|c|c|c|}
% \hline
% \multirow{2}{*}{}  & \multicolumn{2}{c|}{Qualitative reachability}                                                                                        & \multicolumn{2}{c|}{Quantitative reachability}                                                     \\ \cline{2-5} 
%                    & NE                                         & SPE                                                                                     & NE                            & SPE                                                                \\ \hline 
% NP-complet         & $\times$ \cite{Bruyere17} &                                                                                         & $\times$                      &                                                                    \\ \hline
% PSPACE-complet     &                                            & $\times$ \cite{DBLP:journals/corr/abs-1809-03888}                      &                               & $\times$ \cite{DBLP:journals/corr/abs-1905.00784} \\ \hline
% Polynomial memory  & \multicolumn{1}{l|}{$\times$}              & \multicolumn{1}{l|}{}                                                                   & \multicolumn{1}{l|}{$\times$} & \multicolumn{1}{l|}{}                                              \\ \hline
% Exponential memory & \multicolumn{1}{l|}{}                      & \multicolumn{1}{l|}{$\times$ \cite{DBLP:journals/corr/abs-1809-03888}} & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{$\times$}                                      \\ \hline
% \end{tabular}}
% \end{table}


%\paragraph{Quantitative reachability games}

%Let us first focus on the componentwise constrained existence of Nash equilibrium in quantitative reachability game.


\begin{theorem}
	\label{thm:quantNEThreshold}
	Let $(\mathcal{G},v_0)$ be a quantitative reachability game. 
	\begin{itemize}
		\item For NE/SPE, Problem~\ref{prob:decisionThreshold} is NP-complete.
		\item If the answer to this decision problem is affirmative, then there exists a strategy profile $\sigma$ with memory in  $\mathcal{O}((|\Pi|+1)\cdot |V| + |\Pi|)$ which satisfies the constraints. Additionnaly, for quantitative reachability games $\sigma$ is such that $\Cost_i(\outcome{\sigma}{v_0}) \leq |\Pi|\cdot|V|$ if $i \in \Visit(\outcome{\sigma}{v_0})$.
		%\item The strategy profile which satisfies constraints of~\eqref{item:compConstExistProb3} need at most $ \max_{i\in\Pi} \{ \overline{y_i} \mid \overline{y_i} < +\infty \} + |V| + |\Pi|$ memory.
	\end{itemize}
\end{theorem}

Notice that, for the quantitative setting, this result also means that if we want to decide if there exists an NE such that Player $i$ visits his target set (it is like chosing $< +\infty$ for the threshold of Player $i$) it suffies to decide this existence with the threshold $|\Pi| \cdot |V|$ for Player $i$.
\begin{theorem}
	\label{thm:qualNEThreshold}
	Let $(\mathcal{G},v_0)$ be a qualitative reachability game. 
	\begin{itemize}
		\item For NE, Problem~\ref{prob:decisionThreshold} is NP-complete.
		\item If the answer to this decision problem is affirmative, then there exists a strategy profile with memory in  $\mathcal{O}((|\Pi|+1)\cdot |V| + |\Pi|)$ which satisfies the constraints. 
		%\item The strategy profile which satisfies constraints of~\eqref{item:compConstExistProb3} need at most $ \max_{i\in\Pi} \{ \overline{y_i} \mid \overline{y_i} < +\infty \} + |V| + |\Pi|$ memory.
	\end{itemize}
\end{theorem}

The proof of NP-completeness states in Theorem~\ref{thm:quantNEThreshold} is due to Propositions~\ref{prop:compConstNashEasy} and~\ref{prop:compConstNashHard} and we obtain the second part of this result thanks to Corollary~\ref{cor:corCritOut1}. The proof of Theorem~\ref{thm:qualNEThreshold} is discussed at the end of this section. 

\begin{proposition}
	\label{prop:compConstNashEasy}
	Let $(\mathcal{G},v_0)$ be a quantitative reachability game, for NE, Problem~\ref{prob:decisionThreshold} is NP-easy.
\end{proposition}
\begin{proof}
	Let $(\mathcal{G},v_0)$ be a quantitative reachability game and let $y \in (\mathbb{N}\cup\{+\infty\})^{|\Pi|}$ be a threshold. By Corollary~\ref{cor:corCritOut2ConstraintProb}, we know that if there exists an NE $\sigma$ which fullfils the constraints, then there exists an other one such that its outcome is of the form $h\ell^\omega$ with $|h\ell|\leq (|\Pi|+1)\cdot |V| $ and which fullfils the constraints too.\\
	
	 Thus, the NP-algorithm is:\\
		\textbf{Step 1:} Guess a lasso $\rho = h\ell^\omega$ with size at most $(|\Pi|+1)\cdot |V|$ such that $\Visit(\rho)= \Visit(h)$ and verify that $\rho$ is a lasso.\\
		\textbf{Step 2:} Compute $\Cost(\rho)$ and verify that $\Cost(\rho) \leq y$.\\
		\textbf{Step 3:} for each $i \in \Pi$, compute the values in $\mathcal{G}_i$ (useful for the next step).\\
		\textbf{Step 4:} verify that $\rho$ is the outcome of an NE (thanks to Theorem~\ref{thm:critOutcomeNE}): as no new player reaches his target set along $\ell$ and $\ell$ is repeated infinitely often at the end of the outcome, we only have to check that $\rho$ is $\ConstNE$-consistent along $h$. \Al{Détailler plus? vu que la consistance est censée etre sur un chemin infini ? }.\\
\qed
\end{proof}

% \begin{enumerate}
	% \item guess a lasso $\rho = h\ell^\omega$ with size at most $(|\Pi|+1)\cdot |V|$ such that $\Visit(\rho)= \Visit(h)$ and verify that $\rho$ is a lasso;
	% 	\item compute $\Cost(\rho)$ and verify that $\Cost(\rho) \leq y$;
	% 	\item for each $i \in \Pi$, compute the values in $\mathcal{G}_i$ (useful for the next step);
	% 	\item verify that $\rho$ is the outcome of an NE (thanks to Theorem~\ref{thm:critOutcomeNE}): as no new player reaches his target set along $\ell$ and $\ell$ is repeated infinitely often at the end of the outcome, we only have to check that $\rho$ is $\ConstNE$-consistent along $h$. \Al{Détailler plus? vu que la consistance est censée etre sur un chemin infini ? }.
%\end{enumerate}

To obtain the NP-completeness it remains to prove the NP-hardness.

\begin{proposition}
	\label{prop:compConstNashHard}	
	Let $(\mathcal{G},v_0)$ be a quantitative reachability game, Problem~\ref{prob:decisionThreshold} is NP-hard.
\end{proposition}
This proof is based on a polynomial reduction from SAT and is inspired by {\color{red} The complexity of Rational synthesis}. \Al{Expliquer plus?}
\begin{proof}
	To prove this proposition, we give a polynomial reduction from the SAT problem that is NP-complete. Let $X = \{x_1, \ldots, x_m \}$ be the set of variables and $\psi = C_1\wedge\ldots \wedge C_n$ is a Boolean formula in CNF over $X$ and equals to the conjonction of the clauses $C_1, \ldots, C_n$. This problem is to decide if the formula $\psi$ is true. Such a formula is true if there exists a valuation $\mathcal{I} : X \rightarrow \{0,1\}$ such that the valution of $X$ with respect to $\mathcal{I}$ evaluates $\psi$ to true.
	
	We build the following quantitative reachability game $\mathcal{G}_{\psi}= (\mathcal{A}, (\Cost_i)_{i \in \Pi}, (F_i)_{i\in \Pi})$ where $\mathcal{A} = (\Pi, V, E, (V_i)_{i \in \Pi})$:
	\begin{itemize}
		\item the arena $\arena$ is depicted in Figure~\ref{fig:redFormToGame} where the set of players $\Pi = \{1, \ldots, n, n+1 \}$ has $n+1$ players: one by clause (players $1$ to $n$) and an additional one. $V_{n+1}$ is depicted by squared vertices and for all $1 \leq i \leq n$, $V_i = \{P_i \}$;
		\item $F_{n+1} = \{ T_w \}$;
		\item for all $1 \leq i \leq n$, $F_i = \{0_x \mid \neg x \in C_i \} \cup \{ 1_x \mid x \in C_i \}\cup \{ T_\ell \}.$
	\end{itemize}
	
	The game $\mathcal{G}_{\psi}$ can be build from $\psi$ in polynomial time. Let us show that $\psi$ is true if and only if there exists an NE $ \sigma $ in $(\mathcal{G}_\psi,x_1)$ such that $\Cost(\outcome{\sigma}{x_1}) \leq (2m,\ldots,2m,2m +n)$.\\
	
	$(\Rightarrow)$ Suppose that $\psi$ is true. Then there exists $\mathcal{I}: X \rightarrow \{0,1\}$ such that the valuation of $\psi$ with respect to $\mathcal{I}$ evaluates $\psi$ to true.
	
	Let us consider $\sigma$ defined in this way:
	
	\begin{itemize}
		\item for all $hv \in \Hist_{n+1}(x_1)$, $\sigma_{n+1}(hv) = \begin{cases} \mathcal{I}(v) & \text{ if } v = x \text{ with } x \in X \\
		 																		x_{k+1} & \text{ if } v = 0_{x_k} \text{ or } 1_{x_k} \text{with } 0 \leq k \leq m-1 \\
		P_1 & \text{if } v = 0_{x_m} \text{ or } 1_{x_m} \\
		T_\ell & \text{if } v = T_\ell \\
		T_w & \text{if } v = T_w\end{cases}$.
		\item for all $1 \leq i \leq n-1 $ (resp. for $i = n$), for all $hv \in \Hist_i(x_1)$ $\sigma_i(hv) = P_{i+1} $ (resp. $T_w$) if $hv$ is consistent with $\sigma_{n+1}$ and $\sigma_i(hv)= T_\ell$ otherwise. 	
		
	\end{itemize}
	
	We now prove that $\sigma$ is an NE. It is clear that $\outcome{\sigma}{x_1}$ is of the forme $hP_1P_2\ldots P_n T_w^\omega$ and as $\sigma_{n+1}$ corresponds to the valuation $\mathcal{I}$ which evaluates $\psi$ to true, we have that : $\Cost_{n+1}(\outcome{\sigma}{x_1})= 2m+n$ and for all $1\leq i \leq n$, $\Cost_i(\outcome{\sigma}{x_1})\leq 2m$. Obviously Player $n+1$ does not have an incentive to deviate from $\sigma_{n+1}$ because it is a the least cost that he can obtain. For each player $i$ such that $1 \leq i \leq n$, as Player $i$ reaches his target set before he can play, changing his strategy does not change his cost. Thus, no player has a profitable deviation and $\sigma$ is an NE.\\
	
	$(\Leftarrow)$ Suppose that there exists an NE $\sigma$ in $(\mathcal{G}_{\psi}, x_1)$ such that $\Cost_i(\outcome{\sigma}{x_1}) \leq (2m, \ldots, 2m, 2m+n)$ and let us prove that $\psi$ is true.
	
	We define $\mathcal{I} : X \rightarrow \{0,1\}$ as follows: for $x \in X$, $\mathcal{I}(x) = \sigma_{n+1}(hx)$ with $hx$ a prefix of $\outcome{\sigma}{x_1}$. Let us show that the valuation $\mathcal{I}$ evaluates $\psi$ to true. For all $1 \leq i \leq n$, $\Cost_i(\outcome{\sigma}{x_1}) \leq 2m$, it means that Player $i$ reaches his target set but not $T_\ell$. Indeed, the cost to reach $T_\ell$ is equal to $2m+1$. Thus, he reaches $\{0_x \mid \neg x \in C_i \} \cup \{ 1_x \mid x \in C_i \}$ and this means that the clause $C_i$ is true if each variable in $C_i$ is replaced by its valuation. As it is the case for each clause, the formula $\psi$ is true.
	
	
	\begin{figure}
	
		
		\centering
		\begin{tikzpicture}
			\node[draw] (x1) at (0,0){$x_1$};
			\node[draw] (x10) at (1, 0.5){$0_{x_1}$};
			\node[draw] (x11) at (1, -0.5){$1_{x_1}$};
			
			\draw[->] (x1) to (x10);
			\draw[->] (x1) to (x11);
			
			\node[draw] (x2) at (2,0){$x_2$};
			\node[draw] (x20) at (3,0.5){$0_{x_2}$};
			\node[draw] (x21) at (3,-0.5){$1_{x_2}$};
			
			\draw[->] (x10) to (x2);
			\draw[->] (x11) to (x2);
			\draw[->] (x2) to (x20);
			\draw[->] (x2) to (x21);
			
			\node (int1) at (4,0){\ldots};
			\draw[->] (x20) to (int1);
			\draw[->] (x21) to (int1);
			
			\node[draw] (xm) at (4.5,0){$x_m$};
			\node[draw] (xm0) at (5.5,0.5){$0_{x_m}$};
			\node[draw] (xm1) at (5.5,-0.5){$1_{x_m}$};
			
			\draw[->] (xm) to (xm0);
			\draw[->] (xm) to (xm1);
			
			\node[draw,circle] (P1) at (6.5,0){$P_1$};
			
			\draw[->] (xm1) to (P1);
			\draw[->] (xm0) to (P1);
			
			\node[draw,circle] (P2) at (7.5,0){$P_2$};
			
			\draw[->] (P1) to (P2);
			
			\node (int2) at (8.5,0){$\ldots$};
			\draw[->] (P2) to (int2);
			
			\node[draw,circle] (Pn) at (9.5,0){$P_n$};
			\draw[->] (int2) to (Pn);
			
			\node[draw] (Tw) at (10.5,0){$T_{w}$};
			\draw[->] (Pn) to (Tw);
			
			\draw[->] (Tw) to [loop right] (Tw);
			
			\node[draw] (Tl) at (8,1){$T_{\ell}$};
			
			
			\draw[->] (Tl) to [loop above] (Tl);
			
			\draw[->] (P1) to (Tl);
			\draw[->] (P2) to (Tl);
			\draw[->] (Pn) to (Tl);			
		\end{tikzpicture}
			\caption{Reduction from the formula $\psi$ to the quantitative reachability game $\mathcal{G}_{\psi}$}
			\label{fig:redFormToGame}
	\end{figure}
\end{proof}

Notice that this result remains true even if $G = (V,E)$ is strongly connected. {\color{red} Nathan?}

To conclude results about the threshold existence problem in quantitative reachability games with some remarks about a variant of this problem in this setting.

\begin{remark}
	\label{rem:twoThresholds}
	We may also consider this problem but with an upper and a lower threshold. This problem is also NP-complete but the result about memory is a little bit different. Indeed, the memory depends on the upper bound. If there exists an NE which satisfy the constraints then there exists an other one which satisfies the constraints too but with memory in $\mathcal{O}(\max_{i \in \Pi \mid y_i \neq +\infty} y_i + |V| + |\Pi|)$. The difference is due to the fact that we cannot apply iteratively the procedure (P1) and then procedure (P2) to obtain a lasso as procedure (P1) can decrease the cost of the outcome. So the new outcome could not no longer satisfy the constraints. To solve this problem, we only have to apply procedure (P2) on the outcome of $\sigma$.
\end{remark}

We now give a sketch of proof for the results in the qualitative setting.

\begin{proof}[Sketch of proof of Theorem~\ref{thm:qualNEThreshold}]

It is summarized in~\cite{Bruyere17} that Problem~\ref{prob:decisionThreshold}  for quantitative reachability games is NP-complete for Nash equilibrium. To our knowledge, there is no explicit result about the memory which is needed to satisfy the constraints of this problem. We can find the same kind of result as previously. The characterization of the outcomes of NEs can be used by replacing cost functions by gain functions, inversing the inequality and using values in qualitative coalitional games in place of the quantitative ones. Moreover, as applying procedure (P1) on an outcome does not change the gain in the new outcome, the discussion we did in Remark~\ref{rem:twoThresholds} is not needed in this case. Thus, we can use exactly the same arguments  as before to state that if there exists an NE which satisfies the constraints then there exists an other one which satisfies the constraints too but with memory in $\mathcal{O}((|\Pi|+1)\cdot |V| + |\Pi|)$. \qed
\end{proof}

==> sv-paretoOptimality.tex <==
%!TEX root=sv-main.tex

\subsubsection{Pareto-optimal decision problem}


\begin{theorem}
	
	Let $(\mathcal{G},v_0)$ be a quantitative reachability game,
	
	\begin{itemize}
		\item For NE, Problem~\ref{prob:decisionPareto} is NP-hard and belongs to $\Sigma^P_2$.
		\item {\color{red} About memory ???}
	\end{itemize}
\end{theorem}

\begin{theorem}
	
	Let $(\mathcal{G},v_0)$ be a qualitative reachability game,
	
	\begin{itemize}
		\item For NE, Problem~\ref{prob:decisionPareto} is NP-hard and belongs to $\Sigma^P_2$.
		\item {\color{red} About memory ???}
	\end{itemize}
\end{theorem}

Given a reachability game $(\mathcal{G},v_0)$, in order to prove the upper bound of Problem~\ref{prob:decisionPareto}, we need to know what is the complexity of Problem~\ref{prob:4}. This problem lies in co-NP.

\begin{problem}
	\label{prob:4}
	Given a reachability game $(\mathcal{G},v_0)$ and a lasso $\rho \in \Plays$, we want to decide if $(\CostOrGain_i(\rho))_{i\in\Pi}$ is  Pareto-optimal  in $\Plays(v_0)$.
\end{problem}

\begin{lemma}
	Problem~\ref{prob:4} belongs to coNP for qualitative reachability games.
\end{lemma}
\begin{proof}
	If $\rho$ is not Pareto-optimal, there exists a play $\rho'$ such that $\rho \preceq \rho'$. Moreover, thanks to Lemma~\ref{lem:Lassoes}, one may assume that $\rho'$ is a lasso with size at most $(|\Pi|+1)\cdot |V|$. So, we only have to guess such a lasso $\rho'$ and to verify that $\rho \preceq \rho'$. This can be done in polynomial time. \qed
\end{proof}

\Al{ A priori exactement le même résultat pour quantitative reachability games en inversant les $\succeq$}

\begin{proposition}
		Let $(\mathcal{G},v_0)$ be a qualitative reachability game, for NE, Problem~\ref{prob:decisionPareto} belongs to $\Sigma^P_2$.
\end{proposition}
\begin{proof}
	We can provide the following $\Sigma^P_2$-algorithm for Problem~\ref{prob:decisionPareto}, given an oracle for Problem~\ref{prob:4}:\\
	 \textbf{Step 1:} Guess a play $\rho$ as a lasso of size $(|\Pi|+1)\cdot|V|$.\\
	 \textbf{Step 2:} Check that $(\Gain_i(\rho))_{i\in \Pi}$ is Pareto-optimal in $\Plays(v_0)$ using the oracle for Problem~\ref{prob:4}.\\
	 \textbf{Step 3:} Check that $\rho$ is the outcome of a Nash equilibrium using the characterization.\\
	\qed
\end{proof}

==> sv-resNE.tex <==
%!TEX root=sv-main.tex

\subsection{Results on Nash equilibria}
\label{section:resOnNE}


\subsubsection{Characterization}



 %In~\cite{Bruyere17}, this kind of characterization is stated for a particular class of games. In such games, the cost functions have to be \emph{prefix-linear} but it is not the case for the cost function associated with reachability games. Nevertheless, we can recover easily the same kind of result thanks to Theorem~\ref{thm:critOutcomeNE} and for the seek of completeness we provide the proof of this theorem in Appendix~\ref{app:critereOutNE}. 



%--- Si rho est un lasso alors on peut trouver un EN a memoire finie qui a cet outcome---

% Let us now state that if $\rho$ is a lasso and is $\Val$-consistent, then there exists a Nash equilibrium with finite memory which has $\rho$ as outcome.
% 
% \begin{corollary}
% 	\label{rem:memoryForCritOutcomeNE}
% 	
% 	Let $(\mathcal{G},v_0)$ be a quantitative reachability game and let $\rho = h\ell^\omega \in \Plays(v_0)$ be a lasso, the following assertions are equivalent:
% 	
% 	\begin{enumerate}
% 		\item there exists an NE $\sigma$ with memory in $\mathcal{O}(|h\ell|+|\Pi|)$ and such that $\outcome{\sigma}{v_0}= \rho$; 
% 		\item the play $\rho$ is $\ConstNE$-consistent. 
% 	\end{enumerate}
% \end{corollary}


	% To prove this theorem, we can see that the proof of $1 \Rightarrow 2$ of Theorem~\ref{thm:critOutcomeNE} does not change. For $2 \Rightarrow 1$, as already explained, the main idea is that to define $\sigma$ all player play in a way to obtain $\rho$ as outcome. If someone deviates from this outcome, assume it is Player $i$, everybody plays according to its related positional optimal strategy in $\mathcal{G}_i$, \emph{i.e.,} Player $i$ (resp. Player $j \neq i$) plays according to $\sigma^*_i$ (resp. $\sigma^*_{j,i}$). Thus, intuitively, a player has to remember: \emph{i)} $h\ell$ to know both what he has to play to obtain the right outcome  and if someone has deviated  and \emph{ii)} who has deviated to punish him. The definition of the finite machine which describe $\sigma_i$ is given in Appendix~\ref{app:memoryCritNE}.
	
	

%\begin{corollary}
%	Let $\sigma$ be a Nash equilibrium in a quantitative reachability game $(\mathcal{G},v_0)$,
%	there exists $\tau$ an Nash equilibrium in $(\mathcal{G},v_0)$ such that:
%	\begin{enumerate}
%		\item $\Visit(\outcome{\tau}{v_0}) = \Visit(\outcome{\sigma}{v_0})$;
%		\item for all $i \in \Pi$, $\Cost_i(\outcome{\tau}{v_0}) \leq \Cost_i(\outcome{\sigma}{v_0})$;
%		\item for all $i \in \Pi$, the memory of $\tau_i$ is (at most) $(|\Pi|+1)\cdot |V| + |\Pi|$.
%	\end{enumerate}
%\end{corollary}


% \begin{corollary}
% 	\label{cor:corCritOut1}
% 	Let $\sigma$ be an NE in a quantitative reachability game $(\mathcal{G},v_0)$, then there exists $\tau$ an NE in $(\mathcal{G},v_0)$ such that: \emph{i)} $\outcome{\tau}{v_0}$ is a lasso $h\ell^\omega$ such that $|h\ell|\leq (|\Pi|+1)\cdot |V| $; \emph{ii)} for all $i \in \Visit(\outcome{\tau}{v_0})$, $\Cost_i(\outcome{\tau}{v_0}) \leq  \min \{ \Cost_i(\outcome{\sigma}{v_0}), |\Pi|\cdot |V| \}$ and for all $i \not \in Visit(\outcome{\tau}{v_0})$, $\Cost_i(\outcome{\tau}{v_0}) = \Cost_i(\outcome{\sigma}{v_0})= +\infty$; and \emph{iii)} the memory of $\tau$ is in $\mathcal{O}((|\Pi|+1)\cdot |V| + |\Pi|)$. 		
% \end{corollary}
% 
% \begin{corollary}
% 	\label{cor:corCritOut1}
% 	Let $\sigma$ be an NE in a quantitative reachability game $(\mathcal{G},v_0)$, then there exists $\tau$ an NE in $(\mathcal{G},v_0)$ such that:
% 	\begin{itemize} \item  $\outcome{\tau}{v_0}$ is a lasso $h\ell^\omega$ such that $|h\ell|\leq (|\Pi|+1)\cdot |V| $; 
% 		\item for all $i \in \Visit(\outcome{\tau}{v_0})$, $\Cost_i(\outcome{\tau}{v_0}) \leq  \min \{ \Cost_i(\outcome{\sigma}{v_0}), |\Pi|\cdot |V| \}$ and for all $i \not \in \Visit(\outcome{\tau}{v_0})$, $\Cost_i(\outcome{\tau}{v_0}) = \Cost_i(\outcome{\sigma}{v_0})= +\infty$;
% 		\item  the memory of $\tau$ is in $\mathcal{O}((|\Pi|+1)\cdot |V| + |\Pi|)$. 
% 	\end{itemize}
% \end{corollary}

%Given the outcome of the Nash equilibrium, we transforme it into a lasso by eliminating some unnecessary cycle and then identifying a prefix $h\ell$ such that $\ell$ can be repeated infinitely often (procedures P1 and P2) and then use Corollary~\ref{rem:memoryForCritOutcomeNE}. Formal proof given in Appendix~\ref{app:corCritOut1}.

% The following corollary is a direct consequence of Corollary~\ref{cor:corCritOut1}.




\input{sv-NEcomplexity}

%\input{sv-componentWise}
%\input{sv-socialWelfare}
%\input{sv-paretoOptimality}

==> sv-resSPE.tex <==
%!TEX root=sv-main.tex
\subsection{Results on subgame perfect equilibria}
\label{subsection:SPE}


% $\mathcal{O}(2^{|\Pi|} \cdot |\Pi|\cdot |V|^{(|\Pi|+1)\cdot(|\Pi|+|V|)+1})$.


\subsubsection{Complexity and memory results}



% For the qualitative setting, the same kind of results hold.
% 
% \begin{theorem}[\cite{DBLP:journals/corr/abs-1809-03888}]
% 	\label{thm:qualSPEThreshold}
% 	Let $(\mathcal{G},v_0)$ be a qualitative reachability game,
% 	\begin{itemize}
% 		\item For SPE, Problem~\ref{prob:decisionThreshold} is PSPACE-complete.
% 	\item If the answer of the decision problem is positive, there exists a strategy profile with memory in  $\mathcal{O}(|V|^3\cdot |\Pi| \cdot 2^{3 \cdot |\Pi|})$ which satisfies the constraints.
% 		%\item The strategy profile which satisfies constraints of~\eqref{item:compConstExistProb3} need at most $ \max_{i\in\Pi} \{ \overline{y_i} \mid \overline{y_i} < +\infty \} + |V| + |\Pi|$ memory.
% 	\end{itemize}
% \end{theorem}

\begin{theorem}
	\label{thm:SPEComplexity}
	Let $(\mathcal{G},v_0)$ be a quantitative reachability game and $(\mathcal{X},x_0)$ be its extended game, for SPE:
	Problem~\ref{prob:decisionThreshold},~\ref{prob:decisionWelfare} and~\ref{prob:decisionPareto} are PSPACE-complete.
\end{theorem}

\begin{theorem}
	\label{thm:SPEMemory}	
	Let $(\mathcal{G},v_0)$ be a quantitative reachability game and $(\mathcal{X},x_0)$ be its extended game, for SPE:
	\emph{(i)} for each decision problem, if the answer is positive, there exists a strategy profile $ \sigma$ with memory in  $\mathcal{O}(2^{|\Pi|} \cdot |\Pi|\cdot |V|^{(|\Pi|+1)\cdot(|\Pi|+|V|)+1})$  which satisfies the {\color{red}constraints/the problem}, \emph{(ii)} for Problem~\ref{prob:decisionThreshold}, $\sigma$ is such that: if $i\in \Visit(\outcome{\sigma}{x_0})$, $\Cost_i(\outcome{\sigma}{x_0}) \leq |V| \cdot |\Pi|$ and \emph{(iii)} for Problem~\ref{prob:decisionWelfare}, $\sigma$ is such that: $\sum_{i \in \Visit(\outcome{\sigma}{v_0})} \Cost_i(\outcome{\sigma}{v_0}) \leq |\Pi|^2 \cdot |V|$.
\end{theorem}


%---UN THEOREME POUR CHAQUE PROBLEME
% \begin{theorem}
% 	\label{thm:thrSPEQualQuant}
% 	Let $(\mathcal{G},v_0)$ be a qualitative/quantitative reachability game and $(\mathcal{X},x_0)$ be its extended game,
% 	\begin{itemize}
% 		\item For SPE, (\cite{DBLP:journals/corr/abs-1809-03888},\cite{DBLP:journals/corr/abs-1905.00784}) Problem~\ref{prob:decisionThreshold} is PSPACE-complete.
% 		\item  In the quantitative setting (resp. qualitative), if the answer of the decision problem is positive, there exists a strategy profile $ \sigma$ with memory in  $\mathcal{O}(2^{|\Pi|} \cdot |\Pi|\cdot |V|^{(|\Pi|+1)\cdot(|\Pi|+|V|)+1})$ (resp. $\mathcal{O}(|V|^3\cdot |\Pi| \cdot 2^{3 \cdot |\Pi|})$ \cite{DBLP:journals/corr/abs-1809-03888}) which satisfies the constraints. Additionnaly, in quantitative reachability games, $\sigma$ is such that $\Cost_i(\outcome{\sigma}{x_0}) \leq |V| \cdot |\Pi|$ if $i\in \Visit(\outcome{\sigma}{x_0})$.
% 	\end{itemize}
% \end{theorem}
% \begin{theorem}
% 	\label{thm:SPEWelfare}
% 	Let $(\mathcal{G},v_0)$ be a qualitative/quantitative reachability game and $(\mathcal{X},x_0)$ be its extended game.
% 	\begin{itemize}
% 		\item For SPE, Problem~\ref{prob:decisionWelfare} is PSPACE-complete.
% 		\item  In the quantitative setting (resp. qualitative), if the answer of the decision problem is positive, there exists a strategy profile $ \sigma$ with memory in  $\mathcal{O}(2^{|\Pi|} \cdot |\Pi|\cdot |V|^{(|\Pi|+1)\cdot(|\Pi|+|V|)+1})$ (resp. $\mathcal{O}(|V|^3\cdot |\Pi| \cdot 2^{3 \cdot |\Pi|})$ \cite{DBLP:journals/corr/abs-1809-03888}) which satisfies the constraints. Additionnaly, in quantitative reachability games, $\sigma$ is such that $\sum_{i \in \Visit(\outcome{\sigma}{v_0})} \Cost_i(\outcome{\sigma}{v_0}) \leq |\Pi|^2 \cdot |V|$.		
% 	\end{itemize}
% \end{theorem}
% \begin{theorem}
% 		\label{thm:SPEPopti}
% 	Let $(\mathcal{G},v_0)$ be a qualitative/quantitative  reachability game, and let $(\mathcal{X},x_0)$ be its extended game.
% 		\begin{itemize}
% 			\item For SPE, Problem~\ref{prob:decisionPareto} is PSPACE-complete.
% 			\item In the qualitative setting (resp. quantitative), if the answer to this decision problem is positive, then there exists a strategy profile $\sigma$ with memory in  $\mathcal{O}(2^{|\Pi|} \cdot |\Pi|\cdot |V|^{(|\Pi|+1)\cdot(|\Pi|+|V|)+1})$ (resp. $\mathcal{O}(|V|^3\cdot |\Pi| \cdot 2^{3 \cdot |\Pi|})$ which satisfies the problem.
% 		\end{itemize}
% \end{theorem}










==> sv-socialWelfare.tex <==
%!TEX root=sv-main.tex
\subsubsection{Social welfare decision problem}

%\begin{comment}

%\begin{definition}
%	Comment on préfère deux profils point de vue du social welfare -> ordre lexicographique.
%\end{definition}

%\Vero{Ce problème aura été déplacé dans les préliminaires}

%\begin{problem}
%	Let $(\mathcal{G},v_0)$ be a qualitative or a quantitative reachability game and let $c \in \mathbb{R}\cup \{+\infty\}$ and $k \in \{0, \ldots, |\Pi| \}$ be two thresholds, we consider the two following variant of the problem (\Al{trouver un nom}):
%	\begin{enumerate}
%		\item \textbf{Qualitative case:} We want to decide if there exists an NE (resp. SPE) $\sigma$ such that $|\Visit(\outcome{\sigma}{v_0})| \geq k$.
%		\item \textbf{Quantitative case:} We want to decide if there exists an NE (resp. SPE) $\sigma$ such that $|\Visit(\outcome{\sigma}{v_0})| \geq k$ and $\sum_{i \in \Visit(\outcome{\sigma}{v_0})} \Cost_i(\outcome{\sigma}{v_0}) \leq c $.
%	\end{enumerate}
%\end{problem}

%\Al{revoir la présentation}
%\begin{proposition}
%	Let $\sigma$ be a Nash equilibrium in a quantitative reachability game $(\mathcal{G},v_0)$ and $x \in (\mathbb{R}\cup\{+\infty\})^{|\Pi|}$, 
	
%	here is a list of assertions:
%	\begin{enumerate}
%		\item $\sum_{i\in \Pi}\Cost_i(\outcome{\sigma}{v_0}) \leq \sum_{i\in \Pi} x_i$; \label{cor:constraintMemNE2}
%		\item Variante sur somme sur ceux qui voient + nombre de joueurs qui voient leur objectifs; \label{cor:constraintMemNE3}
%		\item there exists $\tau$ an Nash equilibrium in $(\mathcal{G},v_0)$ with memory (at most) $(|\Pi|+1)\cdot |V| + |\Pi|$ such that
%		$\sum_{i\in \Pi}\Cost_i(\outcome{\tau}{v_0}) \leq \sum_{i\in \Pi} x_i$; \label{cor:constraintMemNE5}
%		\item Variante sur somme sur ceux qui voient + nombre de joueurs qui voient leur objectifs.\label{cor:constraintMemNE6}
%	\end{enumerate}
%	We have that: \eqref{cor:constraintMemNE2} $\Rightarrow$ \eqref{cor:constraintMemNE5} and \eqref{cor:constraintMemNE3} $\Rightarrow$ \eqref{cor:constraintMemNE6}.
%\end{proposition}
%\end{comment}

This section is devoted to prove Theorem~\ref{thm:quantNEWelfare} and Theorem~\ref{thm:qualNEWelfare}.
\begin{theorem}
	\label{thm:quantNEWelfare}
	Let $(\mathcal{G},v_0)$ be a quantitative reachability game. 
	\begin{itemize}
		\item For NE, Problem~\ref{prob:decisionWelfare} is NP-complete.
		\item If the answer to this decision problem is affirmative, then there exists a strategy profile $\sigma$ with memory in  $\mathcal{O}((|\Pi|+1)\cdot |V| + |\Pi|)$ which satisfies the constraints and such $\sum_{i \in \Visit(\outcome{\sigma}{v_0})} \Cost_i(\outcome{\sigma}{v_0}) \leq |\Pi|^2 \cdot |V|$ . {\color{red} OK pour ce deuxieme point pour le social welfare?}
		%\item The strategy profile which satisfies constraints of~\eqref{item:compConstExistProb3} need at most $ \max_{i\in\Pi} \{ \overline{y_i} \mid \overline{y_i} < +\infty \} + |V| + |\Pi|$ memory.
	\end{itemize}
\end{theorem}

\begin{theorem}
	\label{thm:qualNEWelfare}
	Let $(\mathcal{G},v_0)$ be a qualitative reachability game. 
	\begin{itemize}
		\item For NE, Problem~\ref{prob:decisionWelfare} is NP-complete.
		\item If the answer to this decision problem is affirmative, then there exists a strategy profile with memory in  $\mathcal{O}((|\Pi|+1)\cdot |V| + |\Pi|)$ which satisfies the constraints. 
		%\item The strategy profile which satisfies constraints of~\eqref{item:compConstExistProb3} need at most $ \max_{i\in\Pi} \{ \overline{y_i} \mid \overline{y_i} < +\infty \} + |V| + |\Pi|$ memory.
	\end{itemize}
\end{theorem}

As previously, we give details for the quantitative setting and we discuss the qualitative case at the end of this section.\\

\begin{lemma}
	\label{lem:NEwelfare}
	Let $k \in \{0, \ldots, |\Pi| \}$ and $c \in \mathbb{N}\cup \{+\infty \}$ be two thresholds, let $p \in (\mathbb{N}\cup \{+\infty\})^{|\Pi|}$ be a cost profile and let $\sigma$ be a strategy profile. We define $\mathcal{R} = \{ i \in \Pi \mid p_i < +\infty \}$. If $(|\mathcal{R}|, \sum_{i\in \mathcal{R}} p_i) \succeq (k,c)$ and $\Cost(\outcome{\sigma}{v_0}) \leq p$ then $\SW(\outcome{\sigma}{v_0}) \succeq (k,c)$.
\end{lemma}

\begin{proof}
	
	Assume that $(|\mathcal{R}|, \sum_{i\in \mathcal{R}} p_i) \succeq (k,c)$ and $\Cost(\outcome{\sigma}{v_0}) \leq p$. First, if $\Visit(\outcome{\sigma}{v_0}) > |\mathcal{R}|$ then $\SW(\outcome{\sigma}{v_0}) \succeq (|\mathcal{R}|, \sum_{i\in \mathcal{R}} p_i)$ and as the lexicographic ordering is transitive we have: $\SW(\outcome{\sigma}{v_0}) \succeq (k,c)$. Secondly, if $\Visit(\outcome{\sigma}{v_0}) = |\mathcal{R}|$, as $\Cost(\outcome{\sigma}{v_0}) \leq p$ it means that $\sum_{i \in \Visit(\outcome{\sigma}{v_0})} \Cost_i(\outcome{\sigma}{v_0}) \leq \sum_{i \in \mathcal{R}}p_i$ and so $\SW(\outcome{\sigma}{v_0}) \succeq (|\mathcal{R}|, \sum_{i\in \mathcal{R}} p_i)$ and as previously it concludes the proof. \qed
	
\end{proof}




\begin{proof}[Proof of Theorem~\ref{thm:quantNEWelfare}]
	
	Let $(\mathcal{G},v_0)$ be a quantitative reachability game and let $k \in \{0, \ldots, |\Pi| \}$ and $c \in \mathbb{N}\cup \{+\infty \}$ be two thresholds. 
	
	The NP-algorithm works as follows:\\	
	\textbf{Step 1:} Guess $p \in (\mathbb{N}\cup \{+\infty\})^{|\Pi|}$ a cost profile;\\
 	\textbf{Step 2:}Let $\mathcal{R} = \{ i \in \Pi \mid p_i < +\infty \}$ be the set of players who have a finite cost in the cost profile $p$, verify if $(|\mathcal{R}|, \sum_{i \in \mathcal{R}}p_i) \succeq (k,c)$;\\
	\textbf{Step 3:} Verify that there exists an NE $\sigma$ in $(\mathcal{G},v_0)$ such that $\Cost(\outcome{\sigma}{v_0}) \leq p.$\\
	
	Thanks to Theorem~\ref{thm:NEThreshold} and Lemma~\ref{lem:NEwelfare}, this algorithm is an NP-algorithm to solve Problem~\ref{prob:decisionWelfare} for Nash equilibrium. Moreover, if there exists an NE which fullfils the constraints there exists one with a polynomial memory and with costs less or equal to $|\Pi|\cdot|V|$ for players who have visited their target set. This leads to an NE such that the cost sum of the players who have visited their target set is less or equal to $|\Pi|^2\cdot |V|$ and it fullfils the constraints too.\\
	
	The NP-hardness is due to a polynomial reduction from SAT in the same spirit than the one for Problem~\ref{prob:decisionThreshold}. {\color{red} plus de blablabla?} \qed
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:qualNEWelfare}]
	
	Let $(\mathcal{G},v_0)$ be a qualitative reachability game and let $k \in \{0, \ldots, |\Pi| \}$ be a threshold.
	
	 The NP-algorithm works as follows:\\	
		\textbf{Step 1:} Guess $p \in \{0,1\}^{|\Pi|}$ a cost profile;\\
		\textbf{Step 2:} Let $\mathcal{R} = \{ i \in \Pi \mid p_i = 1 \}$ be the set of players who have a cost equal to 1 in the cost profile $p$, verify if $|\mathcal{R}| \geq k$;\\
		\textbf{Step 3:} Verify that there exists an NE $\sigma$ in $(\mathcal{G},v_0)$ such that $\Gain(\outcome{\sigma}{v_0}) \geq p.$\\
	
	As if $\Gain(\outcome{\sigma}{v_0}) \geq p$ then $|\Visit(\outcome{\sigma}{v_0})| \geq |\mathcal{R}| \geq k$, and thanks to Theorem~\ref{thm:NEThreshold}, this algorithm is an NP algorithm to solve Problem~\ref{prob:decisionWelfare} for Nash equilibrium. Moreover, if there exists an NE which fullfils the constraints there exists one with a polynomial memory which fullfils the constraints too.\\
	
	The NP-hardness is due to a polynomial reduction from SAT in the same spirit than the one for Problem~\ref{prob:decisionThreshold}. {\color{red} Vérifier preuve JF ? } \qed
	
\end{proof}

